Correlations and Work Statistics in Critical Quantum Systems

In this dissertation, we analyze equilibrium and out-of-equilibrium quantum phase transitions present in quantum spin-$\frac{1}{2}$ models, using a quantum information approach through quantum correlations and phase space formalism, and a quantum thermodynamic approach through the work statistics formalism.

==> Tex/Frontmatter_cedoc.tex <==
%---------------------------------------------------------------------------%
%->> Frontmatter
%---------------------------------------------------------------------------%
%-
%-> Titlepage
%-
\maketitle
%-
%-> Examining Committee Membership


%---------------------------------------------------------------------------%
\intotoc*{\cleardoublepage}{Dédicace}
\chapter*{Dédicace}
\noindent À mon très cher père, De tous les pères, tu es le meilleur. Tu as été et tu seras toujours
un exemple pour moi par tes qualités humaines, ta persévérance et perfectionnisme. En
témoignage de brut d’années de sacrifices, de sollicitudes, d’encouragement de prières.
Pourriez vous trouver dans ce travail le fruit de toutes vos peines et tous vos efforts. En ce
jour, j’espère réaliser l’un de tes rêves. Aucune dédicace ne saurait exprimer mes respects,
ma reconnaissance et mon profond amour. Puisse Dieu vous préserver et vous procurer
santé et bonheur.\\

\noindent À ma très chère mère, Source inépuisable de tendresse et de patience et de sacrifice.
Ta prière et ta bénédiction m’ont été d’un grand secours tout au long de ma vie. Quoique
je puisse dire et écrire, je ne pourrais exprimer ma grande affection et ma profonde reconnaissance. J’espère ne jamais te décevoir, ni traiter ta confiance et tes sacrifices.Puisse
Dieu tout puissant, te préserver et t’accorder santé, longue vie et bonheur.\\

\noindent
À mes chers frères et sœur, Je vous dédie ce travail en témoignage à notre moments
d’enfance passés et mon estime envers vous. Pour nos rêves partagés et notre lien fraternels.\\

\noindent 
À la mémoire de mes grands parents, Que vous reposiez dans le paradis du seigneur.\\

\noindent
À toutes ma famille maternelle et paternelle, Aucun langage ne saurait exprimer
mon respect et ma considération pour votre soutien et encouragements.


\intotoc*{\cleardoublepage}{Remerciement}% add link to toc
\chapter*{Remerciement}
    Ce travail a été réalisé au sein de la structure de recherche \textbf{Équipe de Science de la Matière et du Rayonnement} sous la direction de Monsieur \textbf{Morad EL BAZ}, Professeur de l’Enseignement Supérieur à la Faculté des Sciences de Rabat, et le co-encadrement de Monsieur \textbf{Steve CAMPBELL}, Expert-Professeur à University College Dublin, Irlande. Je tiens à leur exprimer toute ma reconnaissance pour leur disponibilité et leurs grandes qualités humaines d’écoute et d’attention. Qu’ils sont aussi remerciés pour les nombreux encouragements qu'ils m’ont prodigués.\\
    
    \noindent Je remercie Monsieur \textbf{Yassine HASSOUNI}, Professeur de l’Enseignement Supérieur à la
    Faculté des Sciences de Rabat, président du jury, de m’avoir honoré par sa présence en
    présidant le jury de soutenance de mon doctorat. J’en suis honorée et je lui exprime toute
    ma profonde reconnaissance. \\
    
    \noindent Je remercie également Monsieur \textbf{Hamid EZ-ZAHRAOUY}, Professeur de l’Enseignement Supérieur à la Faculté des Sciences de Rabat, d’avoir accepté de rapporter et examiner cette thèse et de scruter de si près le contenu de ma thèse de doctorat. \\
    \noindent Je remercie Monsieur \textbf{Mohamed AZZOUZ}, Professeur de l’Enseignement Supérieur à l’Université Al Akhawayn à Ifrane, d’avoir accepté de juger mon travail en étant un
    rapporteur et examinateur, et pour l’intérêt qu’il a porté à mon travail.\\
    \noindent J’adresse tous mes remerciements à Monsieur \textbf{Adil BELHAJ}, Professeur Habilité à la Faculté des Sciences de Rabat, de l’honneur qu’il m’a fait en acceptant d’être rapporteur et examinteur de cette thèse. \\
    
    \noindent J’exprime ma gratitude à Monsieur \textbf{Bartłomiej Gardas}, Expert-Professeur à Institute of Theoretical and Applied Informatics, Pologne, qui a bien voulu être accepté de participer à
    ce jury de thèse en qualité d’examinateur.\\
    \noindent Je remercie Monsieur \textbf{Mustapha FAQIR}, Professeur de l’Enseignement Supérieur à l’Université International de Rabat, pour faire partie de ce jury en étant un examinateur.

\intotoc*{\cleardoublepage}{\textbf{Résumé}}% add link to toc
\noindent 
Nous étudions théoriquement les caractéristiques critiques des systèmes quantiques à l'équilibre et hors équilibre, du point de vue de l'information quantique et de la thermodynamique quantique. En particulier, nous nous concentrons sur l'analyse des transitions de phase quantique à l'équilibre à l'aide de mesures théoriques de l'information quantique, telles que : l'intrication, la discorde quantique, la cohérence quantique et la fonction de Wigner. Nous montrons la relation entre eux et leur versalité en révélant les caractéristiques saillantes des systèmes quantiques critiques, tels que : le modèle de Heisenberg et la chaine XXZ. De plus, nous explorons les propriétés d’hors-équilibre des systèmes quantiques critiques, en utilisant l'approche des statistiques de travail de la thermodynamique quantique. Nous nous concentrons sur le modèle LMG où nous montrons comment le travail, l'entropie et l'information se comportent lors du franchissement d'une transition de phase quantique à l'état excité. 

\intotoc*{\cleardoublepage}{Abstract}% add link to toc
\begin{abstract}
We theoretically study the critical characteristics of equilibrium and non-equilibrium quantum systems, from the point of view of quantum information and quantum thermodynamics. In particular, we focus on the analysis of equilibrium quantum phase transitions using quantum-information theoretic measures, such as: entanglement, quantum discord, quantum coherence and the Wigner function. We show the relationship between them and their versatility in revealing the salient features of critical quantum systems, such as: the Heisenberg model and the XXZ chain. Furthermore, we explore non-equilibrium properties of critical quantum systems, using the work statistics approach of quantum thermodynamics. We focus on the LMG model where we show how work, entropy and information behave when crossing an excited-state quantum phase transition. 
\end{abstract}

\intotoc*{\cleardoublepage}{Résumé étendu}
\chapter*{Résumé étendu}
    \noindent L'histoire de la vie, de l'humanité et de la société est marquée par des transitions importantes dans les formes de vie, les écosystèmes et la civilisation. L'évolution de l'univers depuis sa création jusqu'à sa forme actuelle serait passée par plusieurs transitions de phase, du plasma à haute température, dû au Big Bang, à la forme refroidie que nous connaissons aujourd'hui. Par conséquent, les transitions de phase sont une pierre angulaire de la nature et revêtent une grande importance quel que soit le domaine auquel on pourrait s'intéresser. En physique, les systèmes complexes présentent des transitions de phase macroscopiques en conséquence des interactions entre de nombreux composants microscopiques. Cela fait de la transition de phase un phénomène émergent, et tout au long de l'histoire, de nombreuses avancées ont été réalisées afin de saisir l'essence de la façon dont l'émergence des états de la matière se produit.\\
    \noindent Nous analysons, dans cette thèse, les transitions de phase quantiques à l'équilibre et hors-équilibre présentes dans les modèles de spin-$\frac{1}{2}$ quantiques, du point de vue de l'information quantique et de la thermodynamique quantique. Nous donnons un aperçu de la littérature sur les transitions de phase classiques et quantiques. De plus, nous couvrons la théorie de l'information classique et quantique, afin de construire le contexte nécessaire pour étudier les propriétés d'équilibre des systèmes de spin quantiques critiques, en utilisant des mesures théoriques de l'information quantique. Nous appliquons ce formalisme au modèle critique de Heisenberg $XX$, où nous étudions le comportement à longue distance de l'intrication, la discorde quantique, et la cohérence quantique, vis-à-vis des perturbations magnétiques et thermiques. Nous montrons la faiblesse de l'intrication, la robustesse des formes générales de corrélations aux fluctuations thermiques, et la versatilité de ces mesures pour révéler la transition de phase quantique du second ordre. De plus, nous étendons l'étude vers la détection des transitions de phase quantiques d'équilibre dans l'espace des phases, à travers la fonction de Wigner. Tout d'abord, nous discutons la fonction de Wigner pour les systèmes de dimension infinie, avec un accent particulier sur le cas de dimension finie, où nous introduisons les constructions de Wootters et Stratonovich de la fonction de Wigner. Ensuite, nous appliquons ce formalisme pour détecter les caractéristiques critiques des modèles $XY$ et $XXZ$, où nous montrons une formule générale reliant la fonction de Wootters, la fonction de Wigner de Stratonovich et les quantités thermodynamiques des modèles de spin, qui peuvent être appliquées à des modèles simples, systèmes bipartites et multipartites. Cette approche nous permet d'introduire une nouvelle façon de représenter, de détecter et de distinguer les transitions de phase quantique du premier, du second et d'ordre infini. De plus, nous montrons que le phénomène de factorisation dans le modèle $XY$ n'est directement détectable que par des quantités basées sur la racine carrée de la matrice de densité réduite bipartite. Nous établissons que les techniques d'espace de phase fournissent un outil simple et prometteur sur le plan expérimental dans l'étude des systèmes à plusieurs corps et nous discutons leur relation avec les mesures de corrélations quantiques et la cohérence quantique. Enfin, nous nous concentrons sur la thermodynamique quantique des transitions de phase quantiques hors d'équilibre. Après avoir présenté la théorie classique de la thermodynamique, nous discutons son extension vers le régime non-équilibre et aux systemes quantique; ainsi que la théorie des ressources de la thermodynamique et son impact sur la théorie du calcul au niveau classique et quantique. Ensuite, nous nous concentrons sur la statistique de travail à travers une transition de phase quantique à l'état excité qui se manifestant dans la dynamique du modèle Lipkin-Meshkov-Glick, initialisée à l'état fondamental de la phase ferromagnétique, et soumise à une brusque trempe. Nous montrons comment l'information, le travail et l'entropie se comportent tout au long de la transition de phase à l'état excité . Enfin, nous démontrons que des caractéristiques similaires persistent lorsque le système est initialisé dans un état excité et explorons brièvement le comportement des états initiaux dans la phase paramagnétique.\\
    \noindent À la fin nous discutons quelques perspectives, où nous visons l'exploitation des caractéristiques des systèmes quantiques afin de concevoir des technologies quantiques efficaces. En effet, l'intrication et la cohérence quantique ont été utilisées pour traiter efficacement l'information et communiquer en toute sécurité. Récemment, il y a eu une recrudescence de l'extension de la thermodynamique au régime quantique afin de concevoir
machines thermiques quantiques pour surmonter certaines limitations de leurs homologues classiques. Une façon d'y parvenir est de modéliser le fluide de travail par un système quantique critique et de le conduire à travers le point critique. Au niveau des transitions de phase quantiques à l'équilibre, il a été montré que le franchissement d'une transition de phase quantique du second ordre peut améliorer l'efficacité des moteurs thermiques quantiques. Ici, nous nous intéressons à montrer l'impact de la transition de phase quantique à l'état excité sur l'efficacité des moteurs thermiques quantiques. Pour atteindre cet objectif, nous modéliserons le milieu de travail par un modèle LMG, piloté à travers la transition de phase quantique de l'état excité à travers différents protocoles, par ex. conduite adiabatique et non adiabatique.

